On Designing a Machine Learning Based Wireless Link Quality Classifier

Ensuring a reliable communication in wireless networks strictly depends on the effective estimation of the link quality, which is particularly challenging when propagation environment for radio signals significantly varies. In such environments, intelligent algorithms that can provide robust, resilient and adaptive links are being investigated to complement traditional algorithms in maintaining a reliable communication. In this respect, the data-driven link quality estimation (LQE) using machine learning (ML) algorithms is one of the most promising approaches. In this paper, we provide a quantitative evaluation of design decisions taken at each step involved in developing a ML based wireless LQE on a selected, publicly available dataset. Our study shows that, re-sampling to achieve training class balance and feature engineering have a larger impact on the final performance of the LQE than the selection of the ML method on the selected data.

==> figures/figtex2pdf <==
#!/bin/bash
#
# Wrapper for figtex2eps so that it can produce
# pdf output.
# 
# Basically runs figtex2eps on the same fig file, but
# then applies epstopdf to the result.
#
# $Id: figtex2pdf,v 1.3 2003/10/28 18:55:32 berland Exp $
#

function die
{
    echo "$1"
    echo "Exiting..."
    exit
}

# Check if gptex2eps exists in $PATH
which figtex2eps >/dev/null 2>&1 \
    || die " (Error) Could not find 'figtex2eps'. It must be installed for figtex2pdf to work."

figtex2eps -pdf "$@"
